SQUASH: Serverless and Distributed Quantization-based Attributed Vector Similarity Search

Vector similarity search presents significant challenges in terms of scalability for large and high-dimensional datasets, as well as in providing native support for hybrid queries. Serverless computing and cloud functions offer attractive benefits such as elasticity and cost-effectiveness, but are difficult to apply to data-intensive workloads. Jointly addressing these two main challenges, we present SQUASH, the first fully serverless vector search solution with rich support for hybrid queries. It features OSQ, an optimized and highly parallelizable quantization-based approach for vectors and attributes. Its segment-based storage mechanism enables significant compression in resource-constrained settings and offers efficient dimensional extraction operations. SQUASH performs a single distributed pass to guarantee the return of sufficiently many vectors satisfying the filter predicate, achieving high accuracy and avoiding redundant computation for vectors which fail the predicate. A multi-level search workflow is introduced to prune most vectors early to minimize the load on Function-as-a-Service (FaaS) instances. SQUASH is designed to identify and utilize retention of relevant data in re-used runtime containers, which eliminates redundant I/O and reduces costs. Finally, we demonstrate a new tree-based method for rapid FaaS invocation, enabling the bi-directional flow of data via request/response payloads. Experiments comparing SQUASH with state-of-the-art serverless vector search solutions and server-based baselines on vector search benchmarks confirm significant performance improvements at a lower cost.

==> algos/squash-algo-klt.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}

\begin{algorithm}[h]
\begin{algorithmic}[1]
\setstretch{1.1}
\caption{Karhunen-Loève Transform (KLT)}
\label{algo:klt}

\Require Dataset $X \in \mathbb{R}^{N \times d}$ \Comment{\# of samples $N$, dimensionality $d$}
\State $\mu \gets \frac{1}{n} \sum_{i=1}^{n} X[i,:]$
\State $X_{\text{centered}} \gets X - \mu$
\State $\Sigma \gets \frac{1}{n-1} X_{\text{centered}}^\top X_{\text{centered}}^{ }$
\State $[\lambda, v] \gets \Call{EigenvalueDecomposition}{\Sigma}$
\State $\text{sorted\_indices} \gets \Call{ArgSort}{\lambda, \text{desc}}$
\State $v_{\text{sorted}}$ $\gets v[:, \text{sorted\_indices}]$
\State $W \gets v_{\text{sorted}}$ \Comment{\textit{KLT matrix $W \in \mathbb{R}^{d \times d}$}}
\State $Y \gets X_{\text{centered}} \cdot W$ \Comment{\textit{Transformed dataset $Y \in \mathbb{R}^{n \times d}$}}\\
\Return $Y, W$


\end{algorithmic}
\end{algorithm}


==> figs/insert-osq-a.tex <==
\begin{figure}[]{}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/osq10a.pdf}
    \caption{SQ: Individual variables per dimension}
    \label{fig:subfig-osq-a}
\end{figure}

==> figs/insert-osq-b.tex <==
\begin{figure}[]{}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/osq10b.pdf}
    \caption{OSQ: Segments shared by multiple dimensions}
    \label{fig:subfig-osq-b}
\end{figure}

==> figs/insert-pipeline-figure.tex <==
\begin{figure*}[]%[!h]%
\centering  
% \includegraphics[width=0.9\textwidth]{figs/pipeline7_cropped.pdf}
\includegraphics[scale=0.85]{figs/pipeline7_cropped.pdf}
\Description{SQUASH multi-stage search workflow}
\caption{SQUASH multi-stage search workflow}
\label{fig:squash-pipeline}
\end{figure*}
